Thinkback: Task-SpecificOut-of-Distribution Detection

The increased success of Deep Learning (DL) has recently sparked large-scale deployment of DL models in many diverse industry segments. Yet, a crucial weakness of supervised model is the inherent difficulty in handling out-of-distribution samples, i.e., samples belonging to classes that were not presented to the model at training time. We propose in this paper a novel way to formulate the out-of-distribution detection problem, tailored for DL models. Our method does not require fine tuning process on training data, yet is significantly more accurate than the state of the art for out-of-distribution detection.

==> 03_dataset.tex <==


% Traffic Classification
%Our datasets comes from two separate product lines, offering device and services for the \emph{Enterprise campus} and \emph{Customer OLT/ONT} market segments respectively.  In a nutshell the datasets comprise of packet-level captures from 4 real customer deployments, spanning over 1 week each, where individual flows are annotated with labels provided by a commercial-grade engine as we describe next.  

% Image recognition

==> plots/plot.pilot_study.poster_a1.tex <==
% Created by tikzDevice version 0.7.0 on 2016-03-28 15:07:30
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor[named]{fillColor}{rgb}{1.00,1.00,1.00}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (758.83,202.36);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (758.83,202.36);
\definecolor[named]{drawColor}{rgb}{1.00,1.00,1.00}
\definecolor[named]{fillColor}{rgb}{1.00,1.00,1.00}

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round,fill=fillColor] (  0.00,  0.00) rectangle (758.84,202.36);
\end{scope}
\begin{scope}
\path[clip] (150.51, 64.01) rectangle (724.69,188.13);
\definecolor[named]{fillColor}{rgb}{0.92,0.92,0.92}

\path[fill=fillColor] (150.51, 64.01) rectangle (724.69,188.13);
\definecolor[named]{drawColor}{rgb}{1.00,1.00,1.00}

\path[draw=drawColor,line width= 0.3pt,line join=round] (251.18, 64.01) --
	(251.18,188.13);

\path[draw=drawColor,line width= 0.3pt,line join=round] (375.46, 64.01) --
	(375.46,188.13);

\path[draw=drawColor,line width= 0.3pt,line join=round] (499.74, 64.01) --
	(499.74,188.13);

\path[draw=drawColor,line width= 0.3pt,line join=round] (624.02, 64.01) --
	(624.02,188.13);

\path[draw=drawColor,line width= 0.6pt,line join=round] (189.04, 64.01) --
	(189.04,188.13);

\path[draw=drawColor,line width= 0.6pt,line join=round] (313.32, 64.01) --
	(313.32,188.13);

\path[draw=drawColor,line width= 0.6pt,line join=round] (437.60, 64.01) --
	(437.60,188.13);

\path[draw=drawColor,line width= 0.6pt,line join=round] (561.88, 64.01) --
	(561.88,188.13);

\path[draw=drawColor,line width= 0.6pt,line join=round] (686.16, 64.01) --
	(686.16,188.13);
\definecolor[named]{drawColor}{rgb}{0.00,0.00,0.00}
\definecolor[named]{fillColor}{rgb}{0.00,0.00,0.00}

\path[draw=drawColor,line width= 0.6pt,line join=round,fill=fillColor] (437.60, 64.01) -- (437.60,188.13);
\definecolor[named]{fillColor}{rgb}{0.97,0.97,0.97}

\path[fill=fillColor] (437.60, 69.83) rectangle (398.54,104.74);
\definecolor[named]{fillColor}{rgb}{0.57,0.77,0.87}

\path[fill=fillColor] (398.54, 69.83) rectangle (363.03,104.74);
\definecolor[named]{fillColor}{rgb}{0.79,0.00,0.13}

\path[fill=fillColor] (363.03, 69.83) rectangle (359.48,104.74);
\definecolor[named]{fillColor}{rgb}{0.97,0.97,0.97}

\path[fill=fillColor] (437.60,108.61) rectangle (409.19,148.52);
\definecolor[named]{fillColor}{rgb}{0.57,0.77,0.87}

\path[fill=fillColor] (409.19,108.61) rectangle (394.99,148.52);
\definecolor[named]{fillColor}{rgb}{0.97,0.97,0.97}

\path[fill=fillColor] (437.60,147.40) rectangle (391.44,182.31);
\definecolor[named]{fillColor}{rgb}{0.57,0.77,0.87}

\path[fill=fillColor] (391.44,147.40) rectangle (355.93,182.31);
\definecolor[named]{fillColor}{rgb}{0.79,0.00,0.13}

\path[fill=fillColor] (355.93,147.40) rectangle (348.83,182.31);
\definecolor[named]{fillColor}{rgb}{0.97,0.97,0.97}

\path[fill=fillColor] (437.60, 69.83) rectangle (476.66,104.74);
\definecolor[named]{fillColor}{rgb}{0.02,0.44,0.69}

\path[fill=fillColor] (476.66, 69.83) rectangle (565.43,104.74);
\definecolor[named]{fillColor}{rgb}{0.96,0.65,0.51}

\path[fill=fillColor] (565.43, 69.83) rectangle (608.04,104.74);
\definecolor[named]{fillColor}{rgb}{0.97,0.97,0.97}

\path[fill=fillColor] (437.60,108.61) rectangle (466.01,148.52);
\definecolor[named]{fillColor}{rgb}{0.02,0.44,0.69}

\path[fill=fillColor] (466.01,108.61) rectangle (597.39,148.52);
\definecolor[named]{fillColor}{rgb}{0.96,0.65,0.51}

\path[fill=fillColor] (597.39,108.61) rectangle (643.55,148.52);
\definecolor[named]{fillColor}{rgb}{0.97,0.97,0.97}

\path[fill=fillColor] (437.60,147.40) rectangle (483.76,182.31);
\definecolor[named]{fillColor}{rgb}{0.02,0.44,0.69}

\path[fill=fillColor] (483.76,147.40) rectangle (547.68,182.31);
\definecolor[named]{fillColor}{rgb}{0.96,0.65,0.51}

\path[fill=fillColor] (547.68,147.40) rectangle (597.39,182.31);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (758.83,202.36);
\definecolor[named]{drawColor}{rgb}{0.30,0.30,0.30}

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.90] at (145.56,122.97) {Organisation};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.90] at (145.56,161.76) {Timer Feature};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.90] at (145.56, 84.18) {Activity Listing};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (758.83,202.36);
\definecolor[named]{drawColor}{rgb}{0.20,0.20,0.20}

\path[draw=drawColor,line width= 0.6pt,line join=round] (189.04, 61.26) --
	(189.04, 64.01);

\path[draw=drawColor,line width= 0.6pt,line join=round] (313.32, 61.26) --
	(313.32, 64.01);

\path[draw=drawColor,line width= 0.6pt,line join=round] (437.60, 61.26) --
	(437.60, 64.01);

\path[draw=drawColor,line width= 0.6pt,line join=round] (561.88, 61.26) --
	(561.88, 64.01);

\path[draw=drawColor,line width= 0.6pt,line join=round] (686.16, 61.26) --
	(686.16, 64.01);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (758.83,202.36);
\definecolor[named]{drawColor}{rgb}{0.30,0.30,0.30}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.90] at (189.04, 42.86) {100};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.90] at (313.32, 42.86) {50};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.90] at (437.60, 42.86) {0};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.90] at (561.88, 42.86) {50};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.90] at (686.16, 42.86) {100};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (758.83,202.36);
\definecolor[named]{drawColor}{rgb}{0.00,0.00,0.00}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.90] at (437.60, 32.26) {Percentage};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (758.83,202.36);
\definecolor[named]{fillColor}{rgb}{1.00,1.00,1.00}

\path[fill=fillColor] (131.44,  8.54) rectangle (743.76, 21.53);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (758.83,202.36);
\definecolor[named]{drawColor}{rgb}{1.00,1.00,1.00}
\definecolor[named]{fillColor}{rgb}{0.95,0.95,0.95}

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round,fill=fillColor] (139.33, 12.80) rectangle (153.78, 17.26);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (758.83,202.36);
\definecolor[named]{fillColor}{rgb}{0.79,0.00,0.13}

\path[fill=fillColor] (140.04, 8.52) rectangle (153.07, 21.55);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (758.83,202.36);
\definecolor[named]{fillColor}{rgb}{0.79,0.00,0.13}

\path[fill=fillColor] (140.04, 8.52) rectangle (153.07, 21.55);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (758.83,202.36);
\definecolor[named]{drawColor}{rgb}{1.00,1.00,1.00}
\definecolor[named]{fillColor}{rgb}{0.95,0.95,0.95}

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round,fill=fillColor] (309.24, 12.80) rectangle (323.70, 17.26);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (758.83,202.36);
\definecolor[named]{fillColor}{rgb}{0.57,0.77,0.87}

\path[fill=fillColor] (309.95, 8.52) rectangle (322.99, 21.55);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (758.83,202.36);
\definecolor[named]{fillColor}{rgb}{0.57,0.77,0.87}

\path[fill=fillColor] (309.95, 8.52) rectangle (322.99, 21.55);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (758.83,202.36);
\definecolor[named]{drawColor}{rgb}{1.00,1.00,1.00}
\definecolor[named]{fillColor}{rgb}{0.95,0.95,0.95}

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round,fill=fillColor] (404.15, 12.80) rectangle (418.60, 17.26);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (758.83,202.36);
\definecolor[named]{fillColor}{rgb}{0.97,0.97,0.97}

\path[fill=fillColor] (404.86, 8.52) rectangle (417.89, 21.55);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (758.83,202.36);
\definecolor[named]{fillColor}{rgb}{0.97,0.97,0.97}

\path[fill=fillColor] (404.86, 8.52) rectangle (417.89, 21.55);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (758.83,202.36);
\definecolor[named]{drawColor}{rgb}{1.00,1.00,1.00}
\definecolor[named]{fillColor}{rgb}{0.95,0.95,0.95}

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round,fill=fillColor] (495.78, 12.80) rectangle (510.24, 17.26);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (758.83,202.36);
\definecolor[named]{fillColor}{rgb}{0.02,0.44,0.69}

\path[fill=fillColor] (496.49, 8.52) rectangle (509.53, 21.55);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (758.83,202.36);
\definecolor[named]{fillColor}{rgb}{0.02,0.44,0.69}

\path[fill=fillColor] (496.49, 8.52) rectangle (509.53, 21.55);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (758.83,202.36);
\definecolor[named]{drawColor}{rgb}{1.00,1.00,1.00}
\definecolor[named]{fillColor}{rgb}{0.95,0.95,0.95}

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round,fill=fillColor] (570.09, 12.80) rectangle (584.54, 17.26);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (758.83,202.36);
\definecolor[named]{fillColor}{rgb}{0.96,0.65,0.51}

\path[fill=fillColor] (570.80, 8.52) rectangle (583.83, 21.55);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (758.83,202.36);
\definecolor[named]{fillColor}{rgb}{0.96,0.65,0.51}

\path[fill=fillColor] (570.80, 8.52) rectangle (583.83, 21.55);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (758.83,202.36);
\definecolor[named]{drawColor}{rgb}{0.00,0.00,0.00}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.80] at (155.59, 9.28) {Strongly Disagree $\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;$};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (758.83,202.36);
\definecolor[named]{drawColor}{rgb}{0.00,0.00,0.00}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.80] at (325.50, 9.28) {Disagree $\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;$};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (758.83,202.36);
\definecolor[named]{drawColor}{rgb}{0.00,0.00,0.00}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.80] at (420.41, 9.28) {Neutral $\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;$};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (758.83,202.36);
\definecolor[named]{drawColor}{rgb}{0.00,0.00,0.00}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.80] at (512.04, 9.28) {Agree $\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;$};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (758.83,202.36);
\definecolor[named]{drawColor}{rgb}{0.00,0.00,0.00}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.80] at (586.35, 9.28) {Strongly Agree $\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;$};
\end{scope}
\end{tikzpicture}


==> plots/poster-plot-comparative_study-atd_dimensions.tex <==
% Created by tikzDevice version 0.10.1 on 2016-11-21 12:40:05
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (289.08,289.08);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (289.08,289.08);
\definecolor{drawColor}{RGB}{255,255,255}
\definecolor{fillColor}{RGB}{255,255,255}

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round,fill=fillColor] (  0.00, -0.00) rectangle (289.08,289.08);
\end{scope}
\begin{scope}
\path[clip] ( 40.68, 72.13) rectangle (286.23,274.85);
\definecolor{fillColor}{gray}{0.92}

\path[fill=fillColor] ( 40.68, 72.13) rectangle (286.23,274.85);
\definecolor{drawColor}{RGB}{255,255,255}

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 40.68,112.06) --
	(286.23,112.06);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 40.68,173.49) --
	(286.23,173.49);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 40.68,234.92) --
	(286.23,234.92);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 40.68, 81.35) --
	(286.23, 81.35);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 40.68,142.78) --
	(286.23,142.78);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 40.68,204.21) --
	(286.23,204.21);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 40.68,265.64) --
	(286.23,265.64);
\definecolor{drawColor}{RGB}{26,71,111}

\path[draw=drawColor,line width= 1.7pt,line join=round] ( 75.76,171.49) --
	(134.23,185.17) --
	(192.69,174.16) --
	(251.16,189.11);
\definecolor{drawColor}{RGB}{144,53,59}

\path[draw=drawColor,line width= 1.7pt,line join=round] ( 75.76,202.87) --
	(134.23,218.12) --
	(192.69,200.42) --
	(251.16,224.81);
\definecolor{drawColor}{RGB}{26,71,111}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 75.76,171.49) circle (  4.10);
\definecolor{drawColor}{RGB}{144,53,59}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 75.76,202.87) circle (  4.10);
\definecolor{drawColor}{RGB}{26,71,111}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (134.23,185.17) circle (  4.10);
\definecolor{drawColor}{RGB}{144,53,59}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (134.23,218.12) circle (  4.10);
\definecolor{drawColor}{RGB}{26,71,111}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (192.69,174.16) circle (  4.10);
\definecolor{drawColor}{RGB}{144,53,59}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (192.69,200.42) circle (  4.10);
\definecolor{drawColor}{RGB}{26,71,111}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (251.16,189.11) circle (  4.10);
\definecolor{drawColor}{RGB}{144,53,59}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (251.16,224.81) circle (  4.10);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (289.08,289.08);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 35.73, 78.32) {-3};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 35.73,139.75) {-1};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 35.73,201.18) {1};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 35.73,262.61) {3};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (289.08,289.08);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 37.93, 81.35) --
	( 40.68, 81.35);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 37.93,142.78) --
	( 40.68,142.78);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 37.93,204.21) --
	( 40.68,204.21);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 37.93,265.64) --
	( 40.68,265.64);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (289.08,289.08);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 75.76, 61.12) {PQ};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (134.23, 61.12) {HQ-I};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (192.69, 61.12) {HQ-S};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (251.16, 61.12) {ATT};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (289.08,289.08);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.10] at (163.46, 29.15) {Dimensions};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (289.08,289.08);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.10] at ( 19.00,173.49) {Mean Score};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (289.08,289.08);
\definecolor{fillColor}{RGB}{255,255,255}

\path[fill=fillColor] ( 92.33, 19.92) rectangle (234.59, 18.41);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (289.08,289.08);
\definecolor{drawColor}{RGB}{255,255,255}
\definecolor{fillColor}{gray}{0.95}

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round,fill=fillColor] (50.21, 7.18) rectangle (64.67, 17.14);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (289.08,289.08);
\definecolor{drawColor}{RGB}{26,71,111}

\path[draw=drawColor,line width= 1.7pt,line join=round] (51.66, 12.16) -- (63.22, 12.16);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (289.08,289.08);
\definecolor{drawColor}{RGB}{26,71,111}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (57.44, 12.16) circle (  4.10);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (289.08,289.08);
\definecolor{drawColor}{RGB}{255,255,255}
\definecolor{fillColor}{gray}{0.95}

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round,fill=fillColor] (170.78, 7.18) rectangle (185.23, 17.14);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (289.08,289.08);
\definecolor{drawColor}{RGB}{144,53,59}

\path[draw=drawColor,line width= 1.7pt,line join=round] (172.22, 12.16) -- (183.78, 12.16);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (289.08,289.08);
\definecolor{drawColor}{RGB}{144,53,59}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (178.00, 12.16) circle (  4.10);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (289.08,289.08);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.88] at (66.48, 6.13) {PortableApps};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (289.08,289.08);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.88] at (187.04, 6.13) {Workbench};
\end{scope}
\end{tikzpicture}


==> plots/poster-plot-comparative_study-atd_portfolio.tex <==
% Created by tikzDevice version 0.10.1 on 2016-11-21 12:41:48
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (274.63,289.08);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (274.63,289.08);
\definecolor{drawColor}{RGB}{255,255,255}
\definecolor{fillColor}{RGB}{255,255,255}

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round,fill=fillColor] (  0.00,  0.00) rectangle (274.63,289.08);
\end{scope}
\begin{scope}
\path[clip] ( 31.15, 63.87) rectangle (271.78,274.85);
\definecolor{fillColor}{gray}{0.92}

\path[fill=fillColor] ( 31.15, 63.87) rectangle (271.78,274.85);
\definecolor{drawColor}{RGB}{255,255,255}

\path[draw=drawColor,line width= 2.3pt,line join=round] ( 31.15, 73.46) --
	(271.78, 73.46);

\path[draw=drawColor,line width= 2.3pt,line join=round] ( 31.15,137.40) --
	(271.78,137.40);

\path[draw=drawColor,line width= 2.3pt,line join=round] ( 31.15,201.33) --
	(271.78,201.33);

\path[draw=drawColor,line width= 2.3pt,line join=round] ( 31.15,265.26) --
	(271.78,265.26);

\path[draw=drawColor,line width= 2.3pt,line join=round] ( 42.09, 63.87) --
	( 42.09,274.85);

\path[draw=drawColor,line width= 2.3pt,line join=round] (115.01, 63.87) --
	(115.01,274.85);

\path[draw=drawColor,line width= 2.3pt,line join=round] (187.93, 63.87) --
	(187.93,274.85);

\path[draw=drawColor,line width= 2.3pt,line join=round] (260.84, 63.87) --
	(260.84,274.85);
\definecolor{drawColor}{RGB}{26,71,111}
\definecolor{fillColor}{RGB}{26,71,111}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (159.09,166.71) circle (  4.10);
\definecolor{fillColor}{RGB}{144,53,59}

\path[fill=fillColor] (191.44,197.72) --
	(199.65,197.72) --
	(199.65,205.93) --
	(191.44,205.93) --
	cycle;
\definecolor{drawColor}{RGB}{255,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.90] at ( 78.55,102.34) {Superfluous};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.90] at ( 78.55,102.34) {Superfluous};
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.90] at ( 78.55,243.00) {Too};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.90] at ( 78.55,243.00) {Too};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.90] at ( 78.55,230.21) {Self-};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.90] at ( 78.55,230.21) {Self-};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.90] at ( 78.55,217.42) {Oriented};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.90] at ( 78.55,217.42) {Oriented};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.90] at (151.47,236.60) {Self-};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.90] at (151.47,236.60) {Self-};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.90] at (151.47,223.82) {Oriented};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.90] at (151.47,223.82) {Oriented};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.90] at (224.38,115.13) {Too};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.90] at (224.38,115.13) {Too};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.90] at (224.38,102.34) {Task-};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.90] at (224.38,102.34) {Task-};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.90] at (224.38, 89.56) {Oriented};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.90] at (224.38, 89.56) {Oriented};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.90] at (151.47,166.28) {Neutral};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.90] at (151.47,166.28) {Neutral};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.90] at (224.38,172.67) {Task-};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.90] at (224.38,172.67) {Task-};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.90] at (224.38,159.88) {Oriented};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.90] at (224.38,159.88) {Oriented};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.90] at (224.38,230.21) {Desired};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.90] at (224.38,230.21) {Desired};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (274.63,289.08);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.10] at (151.47, 29.15) {Pragmatic Quality (PQ)};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (274.63,289.08);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.10] at ( 19.00,169.36) {Hedonic Quality (HQ)};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (274.63,289.08);
\definecolor{fillColor}{RGB}{255,255,255}

\path[fill=fillColor] ( 80.34, 19.92) rectangle (222.59, 18.41);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (274.63,289.08);
\definecolor{drawColor}{RGB}{255,255,255}
\definecolor{fillColor}{gray}{0.95}

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round,fill=fillColor] ( 38.22, 7.18) rectangle (52.68, 17.14);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (274.63,289.08);
\definecolor{drawColor}{RGB}{26,71,111}
\definecolor{fillColor}{RGB}{26,71,111}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 45.45, 12.16) circle (  4.10);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (274.63,289.08);
\definecolor{drawColor}{RGB}{255,255,255}
\definecolor{fillColor}{gray}{0.95}

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round,fill=fillColor] (158.78, 7.18) rectangle (173.24, 17.14);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (274.63,289.08);
\definecolor{fillColor}{RGB}{144,53,59}

\path[fill=fillColor] (161.91, 8.06) --
	(170.11, 8.06) --
	(170.11, 16.27) --
	(161.91, 16.27) --
	cycle;
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (274.63,289.08);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.88] at (54.48, 6.13) {PortableApps};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (274.63,289.08);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.88] at (175.04, 6.13) {Workbench};
\end{scope}
\end{tikzpicture}


==> plots/poster-plot-comparative_study-time_on_task-all.tex <==
% Created by tikzDevice version 0.10.1 on 2016-11-26 20:41:44
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (289.08,231.26);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (289.08,231.26);
\definecolor{drawColor}{RGB}{255,255,255}
\definecolor{fillColor}{RGB}{255,255,255}

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round,fill=fillColor] (  0.00,  0.00) rectangle (289.08,231.26);
\end{scope}
\begin{scope}
\path[clip] (128.53, 59.33) rectangle (289.08,217.04);
\definecolor{fillColor}{gray}{0.92}

\path[fill=fillColor] (128.53, 59.33) rectangle (289.08,217.04);
\definecolor{drawColor}{RGB}{255,255,255}

\path[draw=drawColor,line width= 0.3pt,line join=round] (150.42, 59.33) --
	(150.42,217.04);

\path[draw=drawColor,line width= 0.3pt,line join=round] (179.61, 59.33) --
	(179.61,217.04);

\path[draw=drawColor,line width= 0.3pt,line join=round] (208.80, 59.33) --
	(208.80,217.04);

\path[draw=drawColor,line width= 0.3pt,line join=round] (237.99, 59.33) --
	(237.99,217.04);

\path[draw=drawColor,line width= 0.3pt,line join=round] (267.19, 59.33) --
	(267.19,217.04);

\path[draw=drawColor,line width= 0.6pt,line join=round] (135.82, 59.33) --
	(135.82,217.04);

\path[draw=drawColor,line width= 0.6pt,line join=round] (165.02, 59.33) --
	(165.02,217.04);

\path[draw=drawColor,line width= 0.6pt,line join=round] (194.21, 59.33) --
	(194.21,217.04);

\path[draw=drawColor,line width= 0.6pt,line join=round] (223.40, 59.33) --
	(223.40,217.04);

\path[draw=drawColor,line width= 0.6pt,line join=round] (252.59, 59.33) --
	(252.59,217.04);

\path[draw=drawColor,line width= 0.6pt,line join=round] (281.78, 59.33) --
	(281.78,217.04);
\definecolor{fillColor}{RGB}{26,71,111}

\path[fill=fillColor] (135.82, 75.46) rectangle (234.14,129.22);

\path[fill=fillColor] (135.82,147.14) rectangle (217.06,200.91);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (153.34, 99.60) {6.74};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (153.34,171.28) {5.57};
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.6pt,line join=round] (268.98, 95.17) --
	(268.98,109.51);

\path[draw=drawColor,line width= 0.6pt,line join=round] (268.98,102.34) --
	(199.30,102.34);

\path[draw=drawColor,line width= 0.6pt,line join=round] (199.30, 95.17) --
	(199.30,109.51);

\path[draw=drawColor,line width= 0.6pt,line join=round] (252.99,166.86) --
	(252.99,181.19);

\path[draw=drawColor,line width= 0.6pt,line join=round] (252.99,174.03) --
	(181.14,174.03);

\path[draw=drawColor,line width= 0.6pt,line join=round] (181.14,166.86) --
	(181.14,181.19);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (289.08,231.26);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at (123.58, 99.31) {PortableApps};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at (123.58,171.00) {Workbench};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (289.08,231.26);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.6pt,line join=round] (135.82, 56.58) --
	(135.82, 59.33);

\path[draw=drawColor,line width= 0.6pt,line join=round] (165.02, 56.58) --
	(165.02, 59.33);

\path[draw=drawColor,line width= 0.6pt,line join=round] (194.21, 56.58) --
	(194.21, 59.33);

\path[draw=drawColor,line width= 0.6pt,line join=round] (223.40, 56.58) --
	(223.40, 59.33);

\path[draw=drawColor,line width= 0.6pt,line join=round] (252.59, 56.58) --
	(252.59, 59.33);

\path[draw=drawColor,line width= 0.6pt,line join=round] (281.78, 56.58) --
	(281.78, 59.33);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (289.08,231.26);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (135.82, 48.32) {0};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (165.02, 48.32) {2};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (194.21, 48.32) {4};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (223.40, 48.32) {6};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (252.59, 48.32) {8};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (281.78, 48.32) {10};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (289.08,231.26);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.10] at (183.80, 11.34) {Mean Task Time (Min)};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (289.08,231.26);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.10] at ( 16.68,138.18) {Technique};
\end{scope}
\end{tikzpicture}


==> plots/poster-plot-guided_study-weighted_workload-task3.tex <==
% Created by tikzDevice version 0.10.1 on 2016-11-26 20:25:17
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (375.80,303.53);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (375.80,303.53);
\definecolor{drawColor}{RGB}{255,255,255}
\definecolor{fillColor}{RGB}{255,255,255}

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round,fill=fillColor] (  0.00,  0.00) rectangle (375.80,303.53);
\end{scope}
\begin{scope}
\path[clip] (164.85, 47.95) rectangle (364.42,289.31);
\definecolor{fillColor}{gray}{0.92}

\path[fill=fillColor] (164.85, 47.95) rectangle (364.42,289.31);
\definecolor{drawColor}{RGB}{255,255,255}

\path[draw=drawColor,line width= 0.3pt,line join=round] (192.07, 47.95) --
	(192.07,289.31);

\path[draw=drawColor,line width= 0.3pt,line join=round] (228.35, 47.95) --
	(228.35,289.31);

\path[draw=drawColor,line width= 0.3pt,line join=round] (264.64, 47.95) --
	(264.64,289.31);

\path[draw=drawColor,line width= 0.3pt,line join=round] (300.92, 47.95) --
	(300.92,289.31);

\path[draw=drawColor,line width= 0.3pt,line join=round] (337.21, 47.95) --
	(337.21,289.31);

\path[draw=drawColor,line width= 0.6pt,line join=round] (173.93, 47.95) --
	(173.93,289.31);

\path[draw=drawColor,line width= 0.6pt,line join=round] (210.21, 47.95) --
	(210.21,289.31);

\path[draw=drawColor,line width= 0.6pt,line join=round] (246.50, 47.95) --
	(246.50,289.31);

\path[draw=drawColor,line width= 0.6pt,line join=round] (282.78, 47.95) --
	(282.78,289.31);

\path[draw=drawColor,line width= 0.6pt,line join=round] (319.07, 47.95) --
	(319.07,289.31);

\path[draw=drawColor,line width= 0.6pt,line join=round] (355.35, 47.95) --
	(355.35,289.31);
\definecolor{fillColor}{RGB}{26,71,111}

\path[fill=fillColor] (173.93, 62.77) rectangle (231.00, 79.84);

\path[fill=fillColor] (173.93, 92.46) rectangle (245.74,128.02);

\path[fill=fillColor] (173.93,130.91) rectangle (223.44,167.42);

\path[fill=fillColor] (173.93,169.60) rectangle (242.34,206.58);

\path[fill=fillColor] (173.93,216.12) rectangle (217.39,237.93);

\path[fill=fillColor] (173.93,254.57) rectangle (241.20,277.33);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (375.80,303.53);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at (159.90, 68.28) {Frustration};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at (159.90,107.20) {Effort};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at (159.90,146.13) {Performance};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at (159.90,185.06) {Temporal Demand};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at (159.90,223.99) {Mental Demand};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at (159.90,262.92) {Physical Demand};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (375.80,303.53);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.6pt,line join=round] (162.10, 71.31) --
	(164.85, 71.31);

\path[draw=drawColor,line width= 0.6pt,line join=round] (162.10,110.24) --
	(164.85,110.24);

\path[draw=drawColor,line width= 0.6pt,line join=round] (162.10,149.16) --
	(164.85,149.16);

\path[draw=drawColor,line width= 0.6pt,line join=round] (162.10,188.09) --
	(164.85,188.09);

\path[draw=drawColor,line width= 0.6pt,line join=round] (162.10,227.02) --
	(164.85,227.02);

\path[draw=drawColor,line width= 0.6pt,line join=round] (162.10,265.95) --
	(164.85,265.95);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (375.80,303.53);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.6pt,line join=round] (173.93, 45.20) --
	(173.93, 47.95);

\path[draw=drawColor,line width= 0.6pt,line join=round] (210.21, 45.20) --
	(210.21, 47.95);

\path[draw=drawColor,line width= 0.6pt,line join=round] (246.50, 45.20) --
	(246.50, 47.95);

\path[draw=drawColor,line width= 0.6pt,line join=round] (282.78, 45.20) --
	(282.78, 47.95);

\path[draw=drawColor,line width= 0.6pt,line join=round] (319.07, 45.20) --
	(319.07, 47.95);

\path[draw=drawColor,line width= 0.6pt,line join=round] (355.35, 45.20) --
	(355.35, 47.95);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (375.80,303.53);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (173.93, 36.94) {0};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (210.21, 36.94) {20};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (246.50, 36.94) {40};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (282.78, 36.94) {60};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (319.07, 36.94) {80};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (355.35, 36.94) {100};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (375.80,303.53);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.10] at (264.64, 9.96) {Mean Raw Rating};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (375.80,303.53);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.10] at ( 23.75,168.63) {NASA-TLX Subscales};
\end{scope}
\end{tikzpicture}


==> related_figure_poster.tex <==

\usetikzlibrary{arrows,shadows,positioning}

\tikzset{
  frame/.style={
    rectangle, draw, 
    text width=6em, text centered,
    minimum height=4em,drop shadow,fill=yellow!40,
    rounded corners,
  },
  line/.style={
    draw, -latex',rounded corners=3mm,
  }
}

\begin{figure}
\centering
\resizebox{\columnwidth}{!}{%

\begin{tikzpicture}[font=\small\sffamily\bfseries,very thick,node distance = 2cm]

\node[inner sep=0pt] (cnn) at (0,0)
    {\includegraphics[width=\textwidth]{plots/ourCNN.pdf}};
\node[frame] (C) at (-5,4) [draw,thick,minimum width=1cm,minimum height=1cm] {Input Preprocessing \cite{Zhang15,Liang17,Lee18}};

\node[frame] (D) at (5,4) [draw,thick,minimum width=1cm,minimum height=1cm] {Loss\\Function\cite{Hassen18}};
\node[frame] (F) at (4,-5) [draw,thick,minimum width=1cm,minimum height=1cm] {Classifier \\ K+1 \cite{Neal2018}};
\node[frame] (K) at (8,4) [draw,thick,minimum width=1cm,minimum height=1cm] {Softmax \cite{Hendrycks2017}\\Energy score \cite{liu2021energybased}};

\node[frame] (B) at (-3,-3.8) [draw,thick,minimum width=1cm,minimum height=1cm] {Autoencoder};
\node[frame] (A) at (0,-5) [draw,thick,minimum width=1cm,minimum height=1cm] {GAN};

%\node[frame] (M) at (3,-4) [draw,thick,minimum width=1cm,minimum height=1cm] {G-OpenMax\cite{Ge17}};
\node[frame] (L) at (0,-3) [draw,thick,minimum width=1cm,minimum height=1cm] {Reconstruction Error}; %\cite{Yoshihashi19}

\node[frame] (I) at (2,4) [draw,thick,minimum width=0.2cm,minimum height=1cm] {OpenMax\\ \cite{Bendale15}};

%\node[frame] (J) at (6.5,-5) [draw,thick,minimum width=2cm,minimum height=1cm] {Mahalanobis\\\cite{Lee18}};
%Magnitude\cite{Dhamija18} 
\node[frame] (G) at (6.5,-4) [draw,thick,minimum width=1cm,minimum height=1cm] {Gradient\\based\cite{Yang2021}};


\path [line] (C) -- node[right,align=left,pos=.5] {Augment\\Input}(-5, 1);
\path [line] (-5, -2) |- (B) ;
\path [line] (B) |- (A) ;
\path [line] (D.350) -- (7, 0) ;
%\path [line] (5,-2) -- (7, -2) ;
\path [line] (K) -- (7, 0) ;
%\path [line] (E) -- (3, -1) ;
\path [line] (B) |- node[right,align=right,pos=.7] {Latent \\[3mm] Repr.} (L) ;
\path [line] (A) -- node[right,align=left,pos=.1] {Generate \\[3mm]Unknowns} (F) ;
%\path [line] (J) -- (2, -1) ;
\path [line] (I) -- (4, 0) ;
%\path [line] (A) -- node[left,align=left,pos=.5] {OpenMax} (M) ;
%\path [line] (F) -- (5,-1) ;

\end{tikzpicture}
} 
 %resizebox
\caption{Synoptic of OOD detection wrt an exemplary convolutional DL model: we classify OOD techniques as either working at the input/output of the DL model, or by requiring  modifications to the inner models.} \label{fig:related}

\end{figure}
